Multimodal Earable Sensing for Human Energy Expenditure Estimation

Energy Expenditure Estimation (EEE) is vital for maintaining weight, managing chronic diseases, achieving fitness goals, and improving overall health and well-being. Gold standard measurements for energy expenditure are expensive and time-consuming, hence limiting utility and adoption. Prior work has used wearable sensors for EEE as a workaround. Moreover, earables (ear-worn sensing devices such as earbuds) have recently emerged as a sub-category of wearables with unique characteristics (i.e., small form factor, high adoption) and positioning on the human body (i.e., robust to motion, high stability, facing thin skin), opening up a novel sensing opportunity. However, earables with multimodal sensors have rarely been used for EEE, with data collected in multiple activity types. Further, it is unknown how earable sensors perform compared to standard wearable sensors worn on other body positions. In this study, using a publicly available dataset gathered from 17 participants, we evaluate the EEE performance using multimodal sensors of earable devices to show that an MAE of 0.5 MET (RMSE = 0.67) can be achieved. Furthermore, we compare the EEE performance of three commercial wearable devices with the earable, demonstrating competitive performance of earables

==> other/config.tex <==
\IEEEoverridecommandlockouts                              % This command is only needed if 
\overrideIEEEmargins                                      % Needed to meet printer requirements.

%In case you encounter the following error:
%Error 1010 The PDF file may be corrupt (unable to open PDF file) OR
%Error 1000 An error occurred while parsing a contents stream. Unable to analyze the PDF file.
%This is a known problem with pdfLaTeX conversion filter. The file cannot be opened with acrobat reader
%Please use one of the alternatives below to circumvent this error by uncommenting one or the other
%\pdfobjcompresslevel=0
%\pdfminorversion=4

% See the \addtolength command later in the file to balance the column lengths
% on the last page of the document

% The following packages can be found on http:\\www.ctan.org
%\usepackage{graphics} % for pdf, bitmapped graphics files
%\usepackage{epsfig} % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed
%\usepackage{amsmath} % assumes amsmath package installed
%\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{color, colortbl}
\definecolor{Gray}{gray}{0.9}
\definecolor{LightGray}{gray}{0.6}
\usepackage[most]{tcolorbox}

% \title{\LARGE \bf
% Preparation of Papers for IEEE Sponsored Conferences \& Symposia*
% }

\title{\LARGE \bf
Earable Sensing for Human Energy Expenditure Estimation
}

\author{Yasith Amarasinghe$^{\dagger}$$^{*}$, Darshana Sandaruwan$^{\dagger}$$^{*}$, Thilina Madusanka$^{\dagger}$$^{*}$, Indika Perera$^{\dagger}$ and Lakmal Meegahapola$^{\ddagger}$}% <-this % stops a space
%\thanks{*This work was not supported by any organization}% <-this % stops a space

\thanks{$^{\dagger}$Yasith Amarasinghe, Darshana Sandaruwan, Thilina Madusanka, and Indika Perera are with the Department of Computer Science and Engineering, University of Moratuwa, Sri Lanka}%

\thanks{$^{*}$Equal contribution.}

\thanks{$^{\ddagger}$Lakmal Meegahapola is with the School of Engineering, EPFL,
Switzerland and the Social Computing Group, Idiap Research Institute, Switzerland. {\small lakmal.meegahapola@epfl.ch}}%
